Intervening With Confidence: Conformal Prescriptive Monitoring of Business Processes

Prescriptive process monitoring methods seek to improve the performance of a process by selectively triggering interventions at runtime (e.g., offering a discount to a customer) to increase the probability of a desired case outcome (e.g., a customer making a purchase). The backbone of a prescriptive process monitoring method is an intervention policy, which determines for which cases and when an intervention should be executed. Existing methods in this field rely on predictive models to define intervention policies; specifically, they consider policies that trigger an intervention when the estimated probability of a negative outcome exceeds a threshold. However, the probabilities computed by a predictive model may come with a high level of uncertainty (low confidence), leading to unnecessary interventions and, thus, wasted effort. This waste is particularly problematic when the resources available to execute interventions are limited. To tackle this shortcoming, this paper proposes an approach to extend existing prescriptive process monitoring methods with so-called conformal predictions, i.e., predictions with confidence guarantees. An empirical evaluation using real-life public datasets shows that conformal predictions enhance the net gain of prescriptive process monitoring methods under limited resources.

==> motivation_example.tex <==
\section{Motivating Example} \label{sec:mex}
In an \textit{order-to-cash} process, a case starts when a customer submits an order to purchase a product. Then a process worker (or employee) verifies the submitted order. If it is valid, the employee starts shipping the requested products and delivers them to the customer. This case ends \textit{desirably} (or $dout$) when the customer receives the package specified in the order on time and pays the required invoice. Conversely, it ends \textit{undesirably} (or $uout$) when the customer does not receive the package on time, and accordingly, the customer creates a complaint. 

%Now consider the classical method of reducing the number of complaints that reflects customer satisfaction. 
A PrPM method would use a predictive model to estimate the probability that a customer will complain. It then feeds this prediction to a policy that triggers interventions, primarily targeting customers with the highest complaint probability. However, this policy may trigger interventions for all cases likely to end undesirably. Assuming that predictions will be continuously generated, even when wholly uncertain or all resources are busy and regardless of the consequences of lower-quality probabilities.

A more appropriate way to approach this problem to make the most profitable of resources is to target customers differently. It is not just to allocate resources to customers with a high probability of complaining but to have a valid prediction, e.g., a\textit{ prediction set ($C$)},  that reveals whether a particular customer will complain or not with a certain confidence, e.g., $C=\{uout\}$. Furthermore, it indicates that the predictive model can not distinguish between $dout$ and $uout$ by retaining both, e.g., $C=\{dout, uout\}$ or not predicting anything, i.e., an empty set ($C=\{\}$). In sync, knowing customers who will complain is half the solution, especially with limited resources; Thus, ensuring that the complaining customer will be persuaded via intervention is necessary to maximize the gain. %In sync, Knowing that the customer will complain is half the solution; Thus, ensuring that the complaining customer will be persuaded via intervention with a sufficiently positive impact is necessary. %At the same time, the customer can be persuaded via interventions with a sufficiently positive impact. %Furthermore, it indicates that the predictive model can not distinguish between desired and undesired outcomes by retaining both in the prediction set or not predicting anything, i.e., an empty set. At the same time, the customer can be persuaded via interventions with a sufficiently positive impact. 
